No-Regret Learning in Bayesian Games

Recent price-of-anarchy analyses of games of complete information suggest that coarse correlated equilibria, which characterize outcomes resulting from no-regret learning dynamics, have near-optimal welfare. This work provides two main technical results that lift this conclusion to games of incomplete information, a.k.a., Bayesian games. First, near-optimal welfare in Bayesian games follows directly from the smoothness-based proof of near-optimal welfare in the same game when the private information is public. Second, no-regret learning dynamics converge to Bayesian coarse correlated equilibrium in these incomplete information games. These results are enabled by interpretation of a Bayesian game as a stochastic game of complete information.

==> 1-bcce.tex <==
% !TEX root=bayes-no-regret.tex


\vsdelete{\begin{remark}In the above definitions we assumed that the space $\Sigma=\A_1^{\V_1}\times\ldots\times \A_n^{\V_n}$ admits probability distributions. This is not always obvious, since this is a space of functions. When the valuation spaces $\V_i$ are finite and probability distributions on the action spaces are well defined, then this is true, and hence in the above and subsequent definitions that involve probability distributions over functions $\A_i^{\V_i}$ we will assume that $\V_i$ is finite. For continuous valuation spaces, the issue is a special case of the problem of defining mixed strategies in extensive form games with infinite information sets and the reader is directed to the classic work of Aumann \cite{Aumann1964} for one approach.
\end{remark}}




